Design of the tertiary optical system for the Large Latin American Millimeter Array radio telescope

Many modern radio telescopes employ an observational strategy that involves maximizing the use of their available spaces (cabins), outfitting them with various receivers at different frequencies to detect incoming signals from the sky simultaneously or individually. The Large Latin American Millimeter Array (LLAMA), is a joint venture between Argentina and Brazil consisting of the installation and operation of a 12-meter aperture Cassegrain telescope. It features three available cabins for instrumentation and plans to install six single-pixel heterodyne receivers, covering different bandwidths in the 30 to 950 GHz window of the electromagnetic spectrum, in its two lateral Nasmyth cabins at different phases of the project. Therefore, it is crucial not only to design a tertiary optical system that couples the antenna beam to those receivers, but also to do it in a scalable way. The primary goal for the design is to simultaneously maximize the antenna efficiency while minimizing optical aberrations for all receivers, both fundamental aspects for the optimal functioning of cutting-edge astronomical instruments. In this paper, we present the entire design process, starting from the quasi-optical approach based on the propagation of a fundamental Gaussian beam mode, continuing with the validation of the design based on physical optics simulations, and ending with a tolerance analysis of the system. As a result of this process, a frequency independent tertiary optical system has been achieved for almost all the receivers, which is expected to provide high optical performance for the radio telescope.

==> CAB-A_B6_Parametros_opticos_disenio_3GBT.tex <==

% table:CAB-A B6 Parámetros ópticos diseño 3GBT

\begin{table}[H]%[h!t]
\caption{QO parameters of B6 for CAB-A configuration.} 
\centering
\scalebox{0.75}{\begin{tabular}{|rccccc|}
\hline
\multicolumn{6}{|c|}{Fundamental GBP CAB-A B6}\\
%\multicolumn{6}{|c|}{CAB-A B6 - diseño 3GBT-}\\
\hline
\hline
Freq. (GHz) & 211 &227 &243 &259 &275 \\
$\omega_{NASS}\, \textrm{(mm)}$ &8.58	&7.97	&7.45	&6.99	&6.58\\
$d_{NASS-TOP PLATE}\, \textrm{(mm)}$ &-14.85	&-14.94	&-15.01	&-15.07	&-15.13\\
$d_{TOP PLATE-M3AB6}\, \textrm{(mm)}$ & \multicolumn{5}{c|}{\textsl{135}}\\
\hline
$f_{M3AB6}\, \textrm{(mm)}$ & \multicolumn{5}{c|}{\textsl{215}}\\
$\theta_{M3AB6}\,\hspace{0.5cm}
 \textrm{(deg)}$ & \multicolumn{5}{c|}{\textsl{43.81}}\\
$R_{IN M3AB6}\, \textrm{(mm)}$	&326.27	&302.27	&282.88	&266.99	&253.79\\
$\omega_{M3AB6}\, \textrm{(mm)}$	&11.67	&11.23	&10.87	&10.56	&10.30\\
$R_{OUT M3AB6}\, \textrm{(mm)}$	&-630.44	&-744.66	&-859.96	&-1104.17	&-1406.55\\
$K_{F\, M3AB6}\, \hspace{1cm}$	&0.99966	&0.99969	&0.99971	&0.99972	&0.99974\\
$K_{CO\, M3AB6}\, \hspace{1cm}$	&0.99932	&0.99937	&0.99941	&0.99944	&0.99947\\
\hline
$\omega_{0 OUT M3AB6}\, \textrm{(mm)}$	&10.53	&10.42	&10.30	&10.19	&10.06\\
$d_{OUT-M3AB6}\, \textrm{(mm)}$ &116.84	&103.92	&90.64	&77.08	&63.33\\
$d_{M3AB6-M2A}\, \textrm{(mm)}$ & \multicolumn{5}{c|}{\textsl{1385}}\\	
\hline
$f_{M2A}\, \textrm{(mm)}$ & \multicolumn{5}{c|}{\textsl{857.4}}\\
$\theta_{M2A}\,\hspace{0.5cm}
 \textrm{(deg)}$ & \multicolumn{5}{c|}{\textsl{45}}\\	
$R_{IN M2A}\, \textrm{(mm)}$ &1315.48	&1333.06	&1350.76	&1368.45	&1386.03\\
$\omega_{M2A}\, \textrm{(mm)}$	&55.52	&52.76	&50.43	&48.43	&46.71\\
$R_{OUT M2A}\, \textrm{(mm)}$ &-2462.21	&-2402.91	&-2347.47	&-2295.88	&-2248.03\\
$K_{F\, M2A}\, \hspace{1cm}$	&0.99948	&0.99953	&0.99957	&0.99960	&0.99963\\
$K_{CO\, M2A}\, \hspace{1cm}$	&0.99895	&0.99905	&0.99914	&0.99920	&0.99926\\
\hline
$\omega_{0 OUT M2A}\, \textrm{(mm)}$ &18.88	&18.01	&17.20	&16.44	&15.74\\
$d_{OUT-M2A}\, \textrm{(mm)}$ &2177.56	&2123.05	&2074.49	&2031.27	&1992.75\\
$d_{M2A-M1A}\, \textrm{(mm)}$ & \multicolumn{5}{c|}{\textsl{3800}}\\	
\hline
$f_{M1A}\, \textrm{(mm)}$ & \multicolumn{5}{c|}{\textsl{590}}\\
$\theta_{M1A}\,\hspace{0.5cm}
 \textrm{(deg)}$ & \multicolumn{5}{c|}{\textsl{45}}\\
$R_{IN M1A}\, \textrm{(mm)}$ &2004.48	&2031.26	&2053.69	&2072.63	&2088.73\\
$\omega_{M1A}\, \textrm{(mm)}$ &43.24	&43.12	&43.02	&42.94	&42.87\\
$R_{OUT-M1A}\, \textrm{(mm)}$ &-836.10	&-831.52	&-827.83	&-824.79	&-822.26\\
$K_{F\, M1A}\, \hspace{1cm}$	&0.99933	&0.99933	&0.99934	&0.99934	&0.99934\\
$K_{CO\, M1A}\, \hspace{1cm}$	&0.99866	&0.99866	&0.99867	&0.99868	&0.99868\\
\hline
$\omega_{CASS}\, \textrm{(mm)}$ &8.58	&7.97	&7.45	&6.99	&6.58\\
$d_{OUT-CASS}\, \textrm{(mm)}$ &803.19	&803.09	&803.01	&802.94	&802.88\\
$\omega_{CASS\,IDEAL}\, \textrm{(mm)}$ &8.51	&7.91	&7.39	&6.93	&6.53\\
$K_{AXIALL}\, \hspace{1cm}$	&0.99994	&0.99994	&0.99994	&0.99994	&0.99994\\
\hline
$d_{M1A-SUB REF}\, \textrm{(mm)}$ & \multicolumn{5}{c|}{\textsl{6685.86}}\\
$R_{IN SUB REF}\, \textrm{(mm)}$ &5887.16	&5886.65	&5886.24	&5885.90	&5885.62\\
$\omega_{SUB REF VERTEX}\, \textrm{(mm)}$ &310.50	&310.49	&310.48	&310.47	&310.47\\
$\omega_{SUB REF RIM}\, \textrm{(mm)}$ &316.37	&316.36	&316.35	&316.34	&316.33 \\
\hline
$K_{TOTAL}\, \hspace{1cm}$	&\textbf{0.99535}& \textbf{0.99558}& \textbf{0.99577}&	\textbf{0.99593}&	\textbf{0.98606}\\
%$T_{e \hspace{0.15cm} SUB REF VERTEX}\, \textrm{(dB)}$ &\textbf{12.67}& \textbf{12.67}& \textbf{12.67}&	\textbf{12.67}&	\textbf{12.67}\\
$T_{e \hspace{0.15cm} SUB REF RIM}\, \textrm{(dB)}$ &\textbf{12.20}& \textbf{12.21}& \textbf{12.21}&	\textbf{12.21}&	\textbf{12.21}\\
$\eta_{APERTURE}\, \textrm{(\%)}$ &\textbf{79.89}& \textbf{79.89}& \textbf{79.89}&	\textbf{79.89}&	\textbf{79.89}\\
\hline
\end{tabular}}
\label{table:CAB-A B6 Parámetros ópticos diseño 3GBT}
\end{table}



==> Mirror_geometrical_parameters_3GBT.tex <==

%Tabla parámetros geométricos de espejos diseño 3GBT


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[H]%[h!t]
\caption{Geometrical parameters of mirrors for LT in Cab-A configuration. Ell.: Ellipsoid , Hyp.: Hyperboloid.}
\centering
\scalebox{0.72}{\begin{tabular}{|c|cccccccccccc|}
\hline
\multicolumn{13}{|c|}{\textbf{MIRROR M1A}}                                                                                                                                                                                                                                                                                                                                                                                                                                   \\
\hline

\begin{tabular}[c]{@{}c@{}}Freq.\\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$R_{in}$ \\(mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$R_{out}$ \\(mm)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}$f$ \\ (mm)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}$\theta_i$\\ (deg)\end{tabular}  &
\begin{tabular}[c]{@{}c@{}}$a$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$A_0$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$e$ \end{tabular} &
\begin{tabular}[c]{@{}c@{}}$b$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$\theta$ \\ (deg)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$\omega_m$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Diam. \\ (mm)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}Mirror \\  \end{tabular} \\ 
\hline



452                          & 809.95                    & 2172.62                   & 590.00                   & 45                            & 1491.29                  & 2318.69                   & 0.777411            & 938.01                   & 110.45  & 42.88                                                                                &277x178 & Ell.                                    \\
\hline

%Espejo M2A
\multicolumn{13}{|c|}{\textbf{MIRROR M2A}}                                                                                                                                                                                                                                                                                                                                                                                                                                   \\
\hline

\begin{tabular}[c]{@{}c@{}}Freq.\\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$R_{in}$ \\(mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$R_{out}$ \\(mm)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}$f$ \\ (mm)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}$\theta_i$\\ (deg)\end{tabular}  &
\begin{tabular}[c]{@{}c@{}}$a$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$A_0$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$e$ \end{tabular} &
\begin{tabular}[c]{@{}c@{}}$b$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$\theta$ \\ (deg)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$\omega_m$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Diam. \\ (mm)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}Mirror \end{tabular} \\ 
\hline


452                          & 1903.26                   & 1560.30                   & 857.40                   & 45                            & 1731.78                  & 2461.08                   & 0.710565            & 1218.54                  & 140.66                                                                                   &37.18  &329x223 & Ell.    \\                                 
\hline

%Espejo M3A
\multicolumn{13}{|c|}{\textbf{MIRROR M3A}}                                                                                                                                                                                                                                                                                                                                                                                                                                   \\
\hline

\begin{tabular}[c]{@{}c@{}}Freq.\\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$R_{in}$ \\(mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$R_{out}$ \\(mm)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}$f$ \\ (mm)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}$\theta_i$\\ (deg)\end{tabular}  &
\begin{tabular}[c]{@{}c@{}}$a$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$A_0$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$e$ \end{tabular} &
\begin{tabular}[c]{@{}c@{}}$b$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$\theta$ \\ (deg)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$\omega_m$ \\ (mm)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Diam. \\ (mm)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}Mirror \end{tabular} \\ 
\hline


243                          & 939.62                    & 278.79                    & 215.00                  & 43.81                         & 609.21                   & 968.95                    & 0.795253            & 369.35                   & 163.29                                          & 10.87        &68x47                                  & Ell.                                     \\
324                          & 6426.44                   & 222.44                    & 215.00                  & 44.515                        & 3324.44                  & 6426.52                   & 0.966557            & 852.56                   & 178.02                                          & 9.71         &60x42                                  & Ell.                                              \\
661                          & -755.76                   & 167.38                    & 215.00                  & 44.515                        & 294.19                   & 776.84                    & 1.320299            & 253.62                   & 76.59                                           & 8.42         &50x35                                  & Hyp.                                     \\
\hline
\end{tabular}}

\label{table:Mirror_geometrical_parameters_3GBT}
\end{table}

==> Noise_temperature_contribution_Cab_A_B6.tex <==

% table:Noise_temperature_contribution_Cab_A_B6

\begin{table}[H]%[h!t]
\caption{Noise temperature contribution for B6 (243\,GHz) in Cab-A.\\
The $T_{phys}$ is 296\,K  and 300\,K inside and outside the antenna respectively and the Accum. power is the accumulated power throughout the optical path. The sub-reflector surrounding temperature is obtained from \cite{ASC}, with the telescope pointing to zenith. Temperatures with subscript $n$ are the noise contribution.} 
\centering
\scalebox{0.7}{\begin{tabular}{|ccccccccccc|}
\hline
& M3A-B6 & Flat 2-B6 &Flat 1-B6 &R Flat &M2A &Encoder (bf) & Encoder (ff) &M1A &Sub-ref. &Primary ref.  \\
$T_{source}$(K) &50 &51.505 &53.027 &54.568 &56.082 &57.601 & 57.683 & 57.743 &59.317 &64.422 \\
$T_{surr}$(K) &296 &296 &296 &296 &296 &296 & 296 & 296 &2.798* &300 \\
$T_{phys}$(K) &296 &296 &296 &296 &296 &296 &296 &296 &300 &300 \\
$\varepsilon$ &0.005 &0.005 &0.005 &0.005 &0.005 &0 &0 &0.005 &0.003 &0.02 \\
$R_{so}$ &0.99993 &0.99988 &0.99982 &0.99990 &0.99989 &0.99977 &0.99983 &0.99973 &0.93578 &0.98586 \\
Accum. power &0.99993 &0.99981 &0.99963 &0.99953 &0.99942 &0.99919 &0.99902 &0.99875 &0.93462 &0.92140 \\
$T_{source,n}$(K) &51.484 &52.991 &54.516 &56.053 &57.568 &57.615 & 57.693 & 59.238 &64.230 &71.262 \\
$T_{surr,n}$(K) &0.0216 &0.0361 &0.0518 &0.0284 &0.0335 &0.0684 & 0.0501 & 0.0794 &0.1920 &4.3037 \\
$T_{Refl,n-out}$(K) &51.505 &53.027 &54.568 &56.082 &57.601 &57.683 &57.743 & 59.317 &64.422 &75.565 \\
$T_{Refl,n-add}$(K) &1.505 &1.522 &1.541 &1.514 &1.520 &0.0820 &0.060 & 1.575 &5.105 &11.143 \\
Noise cont.(\%) &5.89 &5.95 &6.03 &5.92 &5.94 &0.32 &0.23 & 6.16 &19.97 &43.59 \\

\hline
\end{tabular}}
\label{table:Noise_temperature_contribution_Cab_A_B6}
\end{table}



==> Optical_performance_of_the_radiotelescope.tex <==

% table:Optical performance of the radiotelescope

\begin{table}[H]%[h!tb]
\caption{Optical performance of the radiotelescope.}
\centering
\scalebox{0.71}{\begin{tabular}{|ccccccccc|} 
\hline
\multicolumn{9}{|c|}{\textbf{Gaussian beam launched from NASS to sky}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\
Band &\begin{tabular}[c]{@{}c@{}}Freq.\\(GHz)\end{tabular} & Config.             & 
\begin{tabular}[c]{@{}c@{}}Ap. eff\\(\%)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Illum. over\\main refl.(dB)\end{tabular} & \begin{tabular}[c]{@{}c@{}}FWHM (arcsec)\\(Max ; Min)\end{tabular} &  \begin{tabular}[c]{@{}c@{}}Peak (arcsec)\\(Az ; El)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Side lobes (dB)\\(left ; rigth)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Cx-pol\\(dB)\end{tabular}   \\ 
\hline
\hline
&211                                                  
& 
& 78.42                                                           
& 10.77                                                       
& (28.76 ; 28.68)                                               
& (0.47 ; -0.04)                                                    
& (-25.10 ; -24.21)                                                       
& -31.67                                                                                                      \\
B6 &243                                                  
& Cab-A LT    
& 78.70                                                       
& 11.05                                                       
& (24.99 ; 24.95)                                               
& (0.40 ; 0.00)                                                    
& (-25.36 ; -24.30)                                                       
& -32.10
\\  
&275                                                  
&     
& 79.04                                                       
& 11.17                                                       
& (22.06 ; 22.03)                                               
& (0.32 ; 0.04)                                                    
& (-25.40 ; -24.24)                                                       
& -32.54
\\
\hline
&275                                                  
& 
& 79.01                                                           
& 11.15                                                       
& (22.06 ; 22.06)                                               
& (0.03 ; 0.00)                                                    
& (-24.38 ; -25.05)                                                       
& -66.70                                                                                                      \\
B7 &324                                                  
& Cab-A LT    
& 79.39                                                       
& 11.24                                                       
& (18.70 ; 18.69)                                               
& (0.03 ; 0.00)                                                    
& (-24.41 ; -24.92)                                                       
& -67.55
\\  
&373                                                  
&     
& 79.50                                                       
& 11.23                                                       
& (16.23 ; 16.22)                                               
& (0.04 ; 0.00)                                                    
& (-24.61 ; -24.98)                                                       
& -67.96
\\
\hline
&602                                                  
& 
& 79.69                                                           
& 11.27                                                       
& (10.04 ; 10.04)                                               
& (0.09 ; 0.04)                                                    
& (-24.67 ; -24.79)                                                       
& -34.06                                                                                                      \\
B9 &661                                                  
& Cab-A LT    
& 79.67                                                       
& 11.26                                                       
& (9.15 ; 9.14)                                               
& (0.08 ; 0.03)                                                    
& (-24.70 ; -24.88)                                                       
& -34.16
\\  
&720                                                  
&     
& 79.66                                                       
& 11.25                                                       
& (8.40 ; 8.40)                                               
& (0.07 ; 0.02)                                                    
& (-24.72 ; -24.93)                                                       
& -34.23
\\
\hline
\hline
&35                                                  
& 
& 67.88                                                           
& 6.26                                                       
& (171.00 ; 163.80)                                               
& (5.82 ; 0,00)                                                    
& (-20.32 ; -19.37)                                                       
& -30.97                                                                                                      \\
B1 &42,5                                                  
& Cab-B LT    
& 73.81                                                       
& 8.50                                                       
& (144.00 ; 138.00)                                               
& (3.80 ; 0.00)                                                    
& (-21.96 ; -20.35)                                                       
& -29.64
\\  
&52                                                  
&     
& 75.88                                                       
& 10.05                                                       
& (106.80 ; 115.20)                                               
& (1.78 ; 0,00)                                                    
& (-23.19 ; -21.51)                                                       
& -28.87
\\                                                                                          \hline
&67                                                  
& 
& 76.94                                                           
& 11.11                                                       
& (91.52 ; 91.39)                                               
& (0.18 ; 0.00)                                                    
& (-24.53 ; -26.28)                                                       
& -28.69                                                                                                      \\
B2+3 &91                                                  
& Cab-B LT    
& 77.29                                                       
& 11.93                                                       
& (67.89 ; 67.79)                                               
& (-0.12 ; 0.00)                                                    
& (-25.29 ; -26.20)                                                       
& -28.67
\\  
&116                                                  
&     
& 77.34                                                       
& 11.70                                                       
& (52.96 ; 52.93)                                               
& (0.10 ; 0.00)                                                    
& (-24.31 ; -25.68)                                                       
& -28.66
\\
\hline
&163                                                  
& 
& 78.89                                                           
& 11.19                                                       
& (37.22 ; 37.20)                                               
& (-0.14 ; -0.04)                                                    
& (-24.86 ; -24.87)                                                       
& -28.47                                                                                                      \\
B5 &187                                                  
& Cab-B FL/LT    
& 78.87                                                       
& 11.16                                                       
& (32.44 ; 32.43)                                               
& (-0.12 ; -0.04)                                                    
& (-24.89 ; -24.90)                                                       
& -28.48
\\  
&211                                                  
&     
& 78.85                                                       
& 11.16                                                       
& (28.76 ; 28.74)                                               
& (-0.11 ; -0.04)                                                    
& (-24.90 ; -24.92)                                                       
& -28.48
\\
\hline
\hline
&211                                                  
& 
& 78.87                                                           
& 11.20                                                       
& (28.77 ; 28.74)                                               
& (-0.18 ; 0.00)                                                    
& (-25.10 ; -24.78)                                                       
& -28.48                                                                                                      \\
B6 &243                                                  
& Cab-B FL    
& 78.84                                                       
& 11.19                                                       
& (24.98 ; 24.96)                                               
& (-0.16 ; 0.00)                                                    
& (-25.07 ; -24.71)                                                       
& -28.47
\\  
&275                                                  
&     
& 78.85                                                       
& 11.21                                                       
& (22.06 ; 22.06)                                               
& (-0.16 ; 0.00)                                                    
& (-25.05 ; -24.60)                                                       
& -28.47
\\
\hline
&602                                                  
& 
& 78.58                                                           
& 11.25                                                       
& (10.07 ; 10.06)                                               
& (-0.13 ; -0.01)                                                    
& (-25.06 ; -23.70)                                                       
& -28.45                                                                                                      \\
B9 &661                                                  
& Cab-B FL    
& 78.46                                                       
& 11.26                                                       
& (9.17 ; 9.17)                                               
& (-0.13 ; -0.01)                                                    
& (-24.47 ; -23.51)                                                       
& -28.45
\\  
&720                                                  
&     
& 78.31                                                       
& 11.27                                                       
& (8.42 ; 8.42)                                               
& (-0.13 ; -0.01)                                                    
& (-24.34 ; -23.31)                                                       
& -28.44
\\
\hline
\end{tabular}}
\label{table:Optical_performance_of_the_radiotelescope}
\end{table}







==> Optical_performance_of_the_tertiary_system.tex <==

% table:Optical performance of the tertiary system

\begin{table}[H]%[h!tb]
\caption{Optical performance of the tertiary system.}
\centering
\scalebox{0.69}{\begin{tabular}{|cccccccccccc|} 
\hline
\multicolumn{12}{|c|}{\textbf{Gaussian beam launched from CASS to NASS}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\
Band             & \begin{tabular}[c]{@{}c@{}}Freq.\\(GHz)\end{tabular} & Config.  & \begin{tabular}[c]{@{}c@{}}Beam \\coupling(\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Gaussicity\\(\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\omega_{0x}$\\(mm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\omega_{0y}$\\(mm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\omega_{0expect}$\\(mm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$x_{offset}$\\(mm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$y_{offset}$\\(mm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Ellipticity\\(\%)\end{tabular}& \begin{tabular}[c]{@{}c@{}}Cx-pol\\(dB)\end{tabular}  \\ 
\hline
\hline
&211                                                  &     & 99.74                                                                                                      & 99.75                                                    & 8.54                                                       & 8.55                                                       & 8.51                                                              & -0.0672                                                    & 0.0048                                                     & 0.16 & -29.48                                                   \\
B6 & 
243                                                  & Cab-A LT    & 99.80                                                                                                      & 99.81                                                    & 7.42                                                       & 7.42                                                       & 7.39                                                              & -0.0478                                                    & 0.0261                                                     & 0.01 & -30.20\\  
&275                                                  &     & 99.83                                                                                                      & 99.84                                                    & 6.56                                                       & 6.56                                                       & 6.53                                                              & -0.0339                                                    & 0.0405                                                     & 0.06 & -30.72\\
\hline
&275                                                  &     & 99.81                                                                                                      & 99.81                                                    & 6.57                                                       & 6.56                                                       & 6.53                                                              & -0.0257                                                    & 0.0000                                                      & 0.13 & -58.02                                                   \\
B7 &324                                                  & Cab-A LT     & 99.86                                                                                                      & 99.86                                                    & 5.57                                                       & 5.56                                                       & 5.54                                                              & -0.0304                                                    & 0.0000                                                      & 0.16 & -61.36\\  
&373                                                  &     & 99.88                                                                                                      & 99.88                                                    & 4.84                                                       & 4.83                                                       & 4.81                                                              & -0.0319                                                     & 0.0000                                                  & 0.18 & -62.15\\
\hline
&602                                                  &     & 99.88                                                                                                      & 99.88                                                    & 3.00                                                       & 3.00                                                       & 2.98                                                              & 0.0080                                                    & 0.0084                                                      & 0.10 & -32.25                                                   \\
B9 &661                                                  & Cab-A LT    & 99.88                                                                                                      & 99.89                                                    & 2.73                                                       & 2.73                                                       & 2.72                                                              & 0.0100                                                    & 0.0054                                                      & 0.08 & -32.36\\  
&720                                                  &     & 99.88                                                                                                      & 99.89                                                    & 2.51                                                       & 2.51                                                       & 2.49                                                              & 0.0115                                                    & 0.0031                                                      & 0.10 & -32.47\\
\hline
\hline
&35                                                  &  & 98.81                                                                                                      & 99.01                                                    & 48.86                                                       & 50.41                                                       & 50.76                                                              & 1.1284                                                    & 0.0780                                                      & 3.17 & -26.73                                                   \\
B1 &42.5                                                  & Cab-B LT       & 99.45                                                                                                      & 99.51                                                    & 42.55                                                       & 43.57                                                       & 42.54                                                              & 0.7730                                                    & 0.0209                                                      & 2.41 & -26.90\\  
&52                                                  &     & 99.78                                                                                                      & 99.78                                                    & 35.07                                                       & 35.48                                                       & 34.82                                                              & 0.0400                                                    & 0.0026                                                                                                       & 1.17 & -27.11\\                                                                                                                                                                                                      \hline
&67                                                  &     & 99.88                                                                                                      & 99.90                                                    & 27.87                                                       & 27.73                                                       & 27.39                                                              & 0.2416                                                    & 0.0000                                                     & 0.49 & -27.26                                                   \\
B2+3 &91                                                  & Cab-B LT    & 99.85                                                                                                      & 99.89                                                    & 20.97                                                       & 20.88                                                       & 20.70                                                              & 0.0366                                                    & 0.0000                                                                                                       & 0.46 & -27.41\\  
&116                                                  &     & 99.84                                                                                                      & 99.87                                                    & 16.30                                                       & 16.24                                                       & 16.12                                                              & 0.0233                                                    & 0.0000                                                      & 0.39 & -27.28\\
\hline
&163                                                  &     & 99.82                                                                                                      & 99.83                                                    & 11.17                                                       & 11.12                                                       & 11.02                                                              & 0.0252                                                    & 0.0145                                                      & 0.45 & -26.96                                                   \\
B5 &187                                                  & Cab-B FL/LT    & 99.81                                                                                                      & 99.82                                                    & 9.74                                                       & 9.71                                                       & 9.60                                                              & 0.0257                                                    & 0.0150                                                      & 0.31 & -26.96\\  
&211                                                  &     & 99.81                                                                                                      & 99.82                                                    & 8.63                                                       & 8.60                                                       & 8.51                                                              & 0.0260                                                    & 0.0153                                                      & 0.35 & -26.95\\
\hline
\hline
&211                                                  &     & 99.60                                                                                                      & 99.62                                                    & 8.66                                                       & 8.63                                                       & 8.51                                                              & 0.0548                                                    & 0.0000                                                      & 0.36 & -26.95                                                   \\
B6 &243                                                  & Cab-B FL    & 99.51                                                                                                      & 99.53                                                    & 7.53                                                       & 7.51                                                       & 7.39                                                              & 0.0543                                                    & 0.0000                                                      & 0.35 & -26.94\\  
&275                                                  &     & 99.41                                                                                                      & 99.44                                                    & 6.67                                                       & 6.64                                                       & 6.53                                                              & 0.0542                                                    & 0.0000                                                      & 0.35 & -26.94\\
\hline
&602                                                  &     & 98.07                                                                                                      & 98.10                                                    & 3.12                                                       & 3.12                                                       & 2.98                                                              & 0.0268                                                    & 0.0051                                                      & 0.19 & -26.93                                                   \\
B9 &661                                                  & Cab-B FL    & 97.71                                                                                                      & 97.74                                                    & 2.86                                                       & 2.86                                                       & 2.72                                                              & 0.0269                                                    & 0.0050                                                      & 0.17 & -26.96\\  
&720                                                  &     & 97.32                                                                                                      & 97.36                                                    & 2.65                                                       & 2.64                                                       & 2.49                                                              & 0.0271                                                    & 0.0049                                                      & 0.15 & -26.93\\
\hline
\end{tabular}}
\label{table:Optical_performance_of_the_tertiary_system}
\end{table}



